Finetune like you pretrain: Improved finetuning of zero-shot vision models

Finetuning image-text models such as CLIP achieves state-of-the-art accuracies on a variety of benchmarks. However, recent works like WiseFT (Wortsman et al., 2021) and LP-FT (Kumar et al., 2022) have shown that even subtle differences in the finetuning process can lead to surprisingly large differences in the final performance, both for in-distribution (ID) and out-of-distribution (OOD) data. In this work, we show that a natural and simple approach of mimicking contrastive pretraining consistently outperforms alternative finetuning approaches. Specifically, we cast downstream class labels as text prompts and continue optimizing the contrastive loss between image embeddings and class-descriptive prompt embeddings (contrastive finetuning). Our method consistently outperforms baselines across 7 distribution shifts, 6 transfer learning, and 3 few-shot learning benchmarks. On WILDS-iWILDCam, our proposed approach FLYP outperforms the top of the leaderboard by $2.3\%$ ID and $2.7\%$ OOD, giving the highest reported accuracy. Averaged across 7 OOD datasets (2 WILDS and 5 ImageNet associated shifts), FLYP gives gains of $4.2\%$ OOD over standard finetuning and outperforms the current state of the art (LP-FT) by more than $1\%$ both ID and OOD. Similarly, on 3 few-shot learning benchmarks, our approach gives gains up to $4.6\%$ over standard finetuning and $4.4\%$ over the state of the art. In total, these benchmarks establish contrastive finetuning as a simple, intuitive, and state-of-the-art approach for supervised finetuning of image-text models like CLIP. Code is available at https://github.com/locuslab/FLYP.

==> ablations.tex <==
\section{Ablation Study}\label{sec:ablations}
\method uses contrastive loss to update both encoders. In this section, we perform several ablations of our proposed approach, which highlight that optimizing the pretraining (contrastive) loss itself is key to the effectiveness of \method.

\subsection{Finetuning both encoders using cross-entropy}
\label{sec:ablations_both_enc_ce}
We first question whether \method is effective simply because it updates both the image and the language encoder, in contrast to standard finetuning approaches, which update only the image encoder using the cross-entropy loss. Our results indicate that the choice of loss function used for finetuning matters indeed.

Let \ours-CE denote a version of our approach where we use the language embeddings (of the text descriptions of class names) as the linear head and optimize both the encoders using cross-entropy (CE) loss.
Formally, given a labeled image $(I,y)$, $\fimg$, $\ftext$ and the $k$ text descriptions for all the classes $\{T_1, T_2, ...T_k\}$, let the class probabilities be given by $\hat{y}\in \R^k$ where $\hat{y}_i=\text{softmax}(\nftext(T_i)^\top\nfimg(I)), \forall i \in [k]$. We then update $\fimg$ and $\ftext$ using gradient descent on $\ell_\text{xent}(\hat{y},y)$, where $\ell_\text{xent}$ denotes the cross-entropy (CE) loss.
% In practice, we implement a batch version.

%Informally, this corresponds to a version of full finetuning (using cross-entropy loss) where the gradients from the linear head flow through the language encoder as well. 

On Imagenet, as shown in Figure~\ref{fig:ablation} (pink curve), \ours-CE performs much worse than \method, which uses the \emph{same} loss as pretraining for updating the encoders. On iWILDCam, \ours-CE is $2\%$ worse ID and $0.6\%$ worse OOD than \ours. Similarly, on other transfer learning datasets, \ours-CE is $1.3\%$ and $1\%$ \emph{worse} in accuracy on PatchCamelyon and Flowers datasets, respectively, compared to \ours. This highlights the fact that the effectiveness of \method is \emph{not} simply due to it finetuning more parameters.

\subsection{\method with frozen language encoder}
\looseness=-1
 Hence, we experiment with a version of \method, where we update \emph{only} the image encoder using the pretraining loss. However, we observe a performance deterioration on both ImageNet (Figure~\ref{fig:ablation}, dark blue curve) and iWILDCam (drop of $2.5\%$ ID and $1.3\%$ OOD) when the language model is frozen.

In Appendix A, we provide additional ablations showing that class-based masking in the minibatch, to avoid class overlap while using the contrastive loss for finetuning, worsens performance.


==> preliminary_old.tex <==
\section{Preliminaries and Notations}\label{sec:preliminary}
\paragraph{Problem Setting}: In this work, our goal is to learn a predictor $f : \mathcal{X} \to [K]$
\begin{enumerate}
    \item (Model) Our goal is to learn a predictor $f : \mathcal{X} \to [K]$ that maps input images $x \in \mathcal{X}$ to outputs $y \in [K]$.
    \item (Distributions) Let $\Pid$ and $\Pood$ denote the underlying distributions over $(x, y)$ in-distribution (ID) and out-of-distribution (OOD) respectively.
    \item (Evaluation metric) We evaluate a model $f$ on the fraction of times it makes a wrong prediction on $\Pid$ and $\Pood$: $\Errid(f) = \E_{x, y \sim \Pid}[\mathbb{I}(f(x) \neq y)]$ and $\Errood(f) = \E_{x, y \sim \Pood}[\mathbb{I}(f(x) \neq y)]$
    \item (Class names) (Motivate why we have class labels, why it helps) $c_k$ denotes the name of class $k \in [K]$ (e.g., `cat', `dog', etc).
    \item (Training data) We have training data $\dtrain = \{(x_i, y_i)\}_{i=1}^{\numtrain}$ sampled i.i.d. from $\Pid$. We only use data from $\Pood$ for evaluation (not for training or hyperparameter selection).
\end{enumerate}

Pretraining:
Image-language models have an image encoder $\f$ and text encoder $\g$. Takes in an image $\iminp$ (e.g., photo of a cat) and corresponding caption $\tinp$ (e.g., ``my pet cat''), and tries to align
\begin{enumerate}
    \item Pretrained im-lang model on $\mathcal{D}_u = \{(\iminp, \tinp)\}_{i=1}^{N_u}$. $\f$ takes in $x$ and gives $\f(x) \in \R^\dembed$. $\g$ take in the corresponding text $t$ and give $\g(t) in \R^\dembed$.
    \item A batch of image-text pairs $B = \{ (\iminp_i, \tinp_i) \}_{i=1}^m$
    \item $\lcont(\f, \g, B) \in \mathbb{R}_{\geq 0}$
    \item $\cont$ is low when each image representation $\f(\iminp_i)$ has high cosine similarity with its corresponding caption representation $\g(\tinp_i)$, and low cosine similarity with captions of other images $\g(\tinp_j)$ where $j \neq i$. The exact form of $L$ is given in Appendix A, and is identical to the CLIP paper (cite).
    \item Write equation, I think it should be in Appendix
    % make $\f(\iminp_i)^\top \g(\tinp_i)$ large for all $i$, and $\f(\iminp_i)^\top \g(\tinp_j)$ low for all $i \neq j$. 
    \item We minimize this loss using minibatch SGD, where we sample batches B from the pretraining data $\mathcal{D}_u$
\end{enumerate}

Baselines:
Zero-shot: We need to define prompts, and zero-shot head.
Linear probe
Fine-tune

Our method: We have our training dataset, and we sample a batch of images $\iminp_1, ..., \iminp_b$. For each image $\iminp_i$ we generate a caption $\tinp_i$ just like in the zero-shot setting, and this gives us a batch of image-caption pairs: 

\begin{enumerate}
    \item Given an image encoder $\f$, text encoder $\g$
    \item Given a train dataset $\dtrain = \{(x_i, y_i)\}_{i=1}^{\numtrain}$, set of templates $T = {\temp_i}_{i=1}^{\numtemp}$
    \item Sample a batch of images $\iminp_1, ..., \iminp_b$
    \item For each $\iminp_i$, select a random caption template $\temp_j \in T$, generate a caption $\tinp_i = \temp_j(c_{y_i})$
    \item This gives us a batch of image-caption pairs: $\{(x_i, y_i)\}$
    \item Just continue pretraining: do a gradient update on $\lcont(\f, \g, B)$
    \item How do we get
\end{enumerate}

Weight ensembling:


In this work, we use \clip~\cite{clip} as the image-text model. Let $\f$ denote the image encoder and $\g$ denote the text encoder of the \clip model.

\subsection{Pre-training of \clip}
Image-text models like CLIP and ALIGN, exploit language supervision for pretraining. Consider access to a large corpus of image-text pairs dataset given by $\mathcal{D}_u = \{(\iminp, \tinp)\}_{i=1}^{N_u}$. Then, \clip minimizes the contrastive loss between the image embeddings $\f(\iminp) \in \R^\dembed$ and text embeddings $\g(\tinp) \in \R^\dembed$ given by:
\begin{equation}
\label{eq:contrastive_loss}
\begin{aligned}
    \lcont(\cdot) & = \sum_{i=1}^{n_u}-log\frac{exp(\simi(\f(\iminp), \g(\tinp))*\tau)}{\sum_{j=1}^{n_u}exp(\simi(\f(\iminp), g_\phi(t_j))*\tau)} \\
    + & \sum_{i=1}^{n_u}-log\frac{exp(\simi(\g(\tinp), \f(\iminp))*\tau)}{\sum_{j=1}^{n_u}exp(\simi(\g(\tinp), f_\theta(x_j))*\tau)},
\end{aligned}
\end{equation}

where $\simi(a, b) = a^Tb/\|a\|\|b\|$ and $\tau$ denotes a learnable temperature scaling parameter.

\subsection{Zero-shot Classification and Finetuning}
\label{sec:zeroshot_head}
Given a $k$ class downstream classification task, a \zeroshot linear head $\hzs \in \R^{d_\text{e}\times k}$ is given by the normalized mean prompt embeddings corresponding to each class. Let $\temp_i(\cdot)$ denote a prompt template (for example,``This is a picture of $\{\cdot\}$'') and $c_j$ denote the classname for the $j^\text{th}$ class. Then the \zeroshot head~\cite{clip} is given as:
\begin{equation}
    \hzs'^j = \frac{1}{N_\text{temp}}\sum_{i=1}^{N_\text{temp}}\frac{\g(\temp_i(c_j))}{\|\g(\temp_i(c_j))\|},\;\;
    \hzs^j = \frac{\hzs'^j}{\|\hzs'^j\|}, \forall j \in [k],
\end{equation}
where $N_\text{temp}$ is the number of prompt templates. The obtained zero-shot linear head (from the text prompts) is then applied to the L2-normalized image embeddings \cite{clip, wiseft}, to get the class probabilities/logits. 

Finally, given a labeled training dataset $\dtrain=\{(x_i,y_i)\}_{i=1}^{N_\text{train}}$ where $x_i \in \R^d$ and $y_i \in \R^k$, typically one learns a classifier $c_\psi : \R^d \rightarrow \R^k$ which minimizes the empirical loss $\left[\ell(c_\psi(x),y)\right]_{(x,y)\sim\dtrain}$. Given a pretrained encoder $\f$, $c_\psi$ is generally parameterized as $c_\psi(x)=\h^T\f(x)$, where $\h$ is a linear head.

Similar to ~\cite{wiseft}, we use the zero-shot head to initialize the linear head for both linear probing and end-to-end finetuning baselines.
% Consider access to a labeled dataset $\mathcal{D}_\text{train}=\{(x_i,y_i)\}_{i=1}^{N_\text{train}}$ for downstream classification, where $x_i \in \R^d$ and $y_i \in \R^k$. Finetuning learns a classifier $c_\psi : \R^d \rightarrow \R^k$, which minimizes the empirical loss $\left[\ell(c_\phi(x),y)\right]_{(x,y)\sim\mathcal{D}_\text{train}}$. Given the pretrained encoder 
% Linear probing then learns a classifier $h: \R^\dembed \rightarrow \R^k$ over the fixed encoder representations $\f(\iminp)\in\R^\dembed$, whereas end-to-end finetuning
\subsection{Weight Ensembling}
WiseFT~\cite{wiseft} observe accuracy gains both in-distribution (ID) and out-of-distribution (OOD), when ensembling the pretrained and the finetuned weights. Specifically, let $\psi_0$ denote the parameters of \zeroshot classifier (with $\hzs$ as the linear head over the pretrained iamge encoder), and let ${\psi_1}$ denote those of finetuned classifier. Then, 
\begin{equation}
    c_\psi^\text{wse}(x, \alpha) = c_{\psi'}(x),\; \text{where } \psi' = (1-\alpha)\psi_0 + \alpha\psi_1 
\end{equation}


